Investigating Vulnerability Disclosures in Open-Source Software Using Bug Bounty Reports and Security Advisories

In the world of open-source software (OSS), the number of known vulnerabilities has tremendously increased. The GitHub Advisory Database contains advisories for security risks in GitHub-hosted OSS projects. As of 09/25/2023, there are 197,609 unreviewed GitHub security advisories. Of those unreviewed, at least 63,852 are publicly documented vulnerabilities, potentially leaving many OSS projects vulnerable. Recently, bug bounty platforms have emerged to focus solely on providing bounties to help secure OSS. In this paper, we conduct an empirical study on 3,798 reviewed GitHub security advisories and 4,033 disclosed OSS bug bounty reports, a perspective that is currently understudied, because they contain comprehensive information about security incidents, e.g., the nature of vulnerabilities, their impact, and how they were resolved. We are the first to determine the explicit process describing how OSS vulnerabilities propagate from security advisories and bug bounty reports, which are the main intermediaries between vulnerability reporters, OSS maintainers, and dependent projects, to vulnerable OSS projects and entries in global vulnerability databases and possibly back. This process uncovers how missing or delayed CVE assignments for OSS vulnerabilities result in projects, both in and out of OSS, not being notified of necessary security updates promptly and corresponding bottlenecks. Based on our findings, we provide suggestions, actionable items, and future research directions to help improve the security posture of OSS projects.

==> content/results.tex <==
\section{Participants}\label{sec:parts}

~\autoref{tab:participants} summarizes participants’ self-reported demographics and experiences. 
We had 80 participants in the listing study and 22 interviewees. Participants were mainly from Europe and North America and were overwhelmingly male. 
This is consistent with other qualitative studies with OSS stakeholders as participants, e.g., ~\cite{liang2022understanding,huang2021fingerprints}.
Further, security experts from industry recommend organizations revisit their security policies and processes at least once a year~\cite{updatesec,updatesec2}, which is consistent with half of our study participants.


\begin{table}[th!]
    \begin{centering}
    \begin{adjustbox}{width=0.48\textwidth}
	\begin{tabular}{llrr}
            \toprule
            \midrule
            \centering
		& & \textbf{L} & \textbf{I} \\ 
		\midrule
            \midrule
		\textbf{Gender}     & Man & 71 & 19   \\
                                & Woman & 6 & 1   \\
                                & Non-binary & 3 & 2  \\
            \midrule
		\textbf{Age}        & 18-29 & 12 & 3  \\
                                & 30-39 & 28 & 8  \\
                                & 40-49 & 32 & 6  \\
                                & 50+ & 8 & 5  \\
		\midrule
		\textbf{Residence}  & Australia & 0 & 0  \\
                                & Africa & 1 & 0  \\
                                & Europe & 39 & 12  \\
                                & Middle East & 3 & 1 \\
                                & North America & 27 & 7  \\
                                & South America & 2 & 1  \\
                                & South Asia & 1 & 0  \\
                                & Southeast Asia & 1 & 0  \\
                                & Other & 6 & 1  \\
		\midrule
		\textbf{Education}  & $\le$ Completed high school & 3 & 1 \\
                                & Trade/technical/vocational & 1 & 1  \\
                                & College, no degree & 8 & 2  \\
                                & Associate’s degree & 1 & 1 \\
                                & Professional degree & 5 & 0  \\
                                & Bachelor's degree & 29 & 8  \\
                                & Graduate degree & 33 & 9 \\
            \midrule
		\textbf{Years working} & < 1 year & 4 & 1  \\
            \textbf{in industry} & 1-5 years & 10 & 2 \\
                                & 5-10 years & 4 & 1  \\
                                & 10+ years & 62 & 18 \\
                                %& None & 4 & 0 \\
            \midrule
		\textbf{Years in OSS} & < 1 year & 1 & 0  \\
            \textbf{maintainence} & 1-5 years & 16 & 4  \\
                                & 5-10 years & 18 & 5   \\
                                & 10+ years & 45 & 13  \\
            \midrule
		\textbf{Has a security} & Yes & 29 & 9  \\
            \textbf{background} & No & 51 & 13  \\
            \midrule
            \textbf{Vulnerabilty} & Every 1-3 months & 10 & 1  \\
		\textbf{management} & Every 6 months & 11 & 3  \\
            \textbf{process review} & Every year & 19 & 4  \\
            \textbf{or update} & Every 2+ years & 8 & 1  \\
            \textbf{frequency} & Never & 32 & 13  \\
            \midrule
		\textbf{OSS project has} & Yes & 31 & 7 \\
            \textbf{funding} & No & 49 & 15  \\
            \midrule
            \midrule
            \textbf{\# of participants} &  & \textbf{80} & \textbf{22}  \\
            \midrule
            \bottomrule
        \end{tabular}
    \end{adjustbox}
    \caption{The number of participants across the two studies along with their respective demographics, various backgrounds, and project details.  Acronyms listed represent, respectively: listing (\textbf{L}) survey study and interview (\textbf{I}) study.}
    \label{tab:participants}
    \end{centering}
\end{table}


In the listing survey and interview studies, our participants are OSS project maintainers who have received and patched vulnerabilities as seen in the GitHub Advisory Database~\cite{gad}. 
We are especially curious about this subset of OSS project maintainers because although they have experience triaging vulnerabilities for projects they own, easily configurable platform security features are generally underused~\cite{ayala2024secfeat}.
%A general breakdown of the 1,920 projects described in Section~\ref{sec:recruit} is shown in~\ref{tab:underuse}.

\section{Results}\label{sec:results}

In the following section, we report and discuss the results for 22 semi-structured interviews with open-source maintainers.
In our reporting, we adhere to the structure of the interview guide shown in~\autoref{fig:flow} from Section~\ref{sec:interviewstudy}.
We report quotes as transcribed with minor grammatical corrections and omissions. e.g., using \textit{``[...]''}, for readability.

We identified \codenums factors from OSS project maintainers, whose projects have a history of vulnerabilities, regarding their vulnerability management efforts using five categories: current practices, general challenges, platform security feature challenges, platform security feature barriers, and platform security feature wants. The curated codes can be found in~\autoref{tab:bigasstable} and list relevant prior work for each code, if applicable. 
 
Our study is closely related to a recent paper that investigated OSS security and trust practices of contributors, owners, and maintainers~\cite{wermke2022qual-OSSP}, i.e., general OSS stakeholders, regardless of vulnerability history or contributions; however,
\textbf{we are the first to investigate vulnerability management challenges that OSS maintainers, whose projects have a history of patched vulnerabilities, face regarding platform security features involving the GitHub Advisory Database}, i.e., by recruiting maintainers whose projects are linked from GitHub security advisories.
This particular perspective is important as OSS project maintainers typically do not have a security background, so learning from maintainers who have a history of vulnerability triaging provides a glimpse of progress towards security-awareness trickling throughout the OSS ecosystem.
Further, using recommended platform security features and practices are key components of transparency and vulnerability awareness, e.g., by publishing security advisories after patching vulnerabilities, for OSS stakeholders. 
We hope to learn more about \textit{how} and \textit{why} such adoption is present, or not, in previously vulnerable projects.

%%%We present how many listing study participants mentioned codes from~\autoref{tab:bigasstable} (\textit{\textbf{L}}) and how many interviewees discussed or argued a particular topic in detail (\textit{\textbf{I}}). 


\input{content/table_nocolors}


\subsection{Current practices used for vulnerability management}\label{sec:currmanagement}

Both of our studies reflect that OSS project maintainers use a variety of tooling both in and out of the GitHub platform.
Most encourage using a private avenue for reporting vulnerabilities while some are okay with using public channels, e.g., GitHub issues, for security bugs. 
Two listing study respondents indicated that they ignore vulnerabilties altogether.

\vspace{0.1cm}

\noindent\textbf{Emails and external tooling or reports }
Using a form of a security contact email or mailing list consisting of project maintainers was the most listed form of current vulnerability management practices ($L=50$, $I=11$). This is consistent with a finding from Wermke et al., where authors identified that having a security contact point was the commonly mentioned aspect of a security policy~\cite{wermke2022qual-OSSP}.

Participants indicated that using email for security reports is sufficient because it discourages reporters from creating a public issue and acts as a private avenue for report resolution ($L=11$, $I=4$), e.g., \textit{``we'll take time to really have a discussion and not just here's my report, okay, I dismiss it or I accept it. It's more like a conversation''} (P4). Others mention having security experts on their maintenance team ($L=3$).% Three interviewees shared a perspective that embodies trust among maintainers:

\leftskip=0.5cm\rightskip=0.5cm

\noindent \textit{``With the projects I've been a part of, we just use one email address everybody can log into, which I suppose is just not a super secure way of managing that point of contact, but we all trust each other as maintainers. We have like a shared password on that email account, and that's just kind of how we do things.''} (P12).

\leftskip=0cm\rightskip=0cm

Listing participants and interviewees also mentioned using tooling outside of GitHub, including internal tools for static analysis ($L=2, I=3$), e.g., Coverity~\cite{coverity}, and receiving external reports from companies ($L=1, I=2$). One interviewee described their relationship with a company that sends bundled vulnerability reports for their OSS project semi-annually:

\leftskip=0.5cm\rightskip=0.5cm

\noindent \textit{``They send me a lot of bugs I never knew about and they give me time to fix it. Once fixed, they publish, and then they come back next year [...] I'm surprised with what they can find, I would like to know why they do that but I never complain. Be grateful, you know?''} (P17).

\leftskip=0cm\rightskip=0cm 

\vspace{0.1cm}

\noindent\textbf{Proactive disclosure process }
Having an established disclosure process after patching vulnerabilities consisting of project maintainers was the second-highest form of current vulnerability management practices ($L=46$, $I=7$). This demonstrates a sense of responsibility within the OSS community since it ensures affected dependent client projects within reach are notified to upgrade~\cite{mohayeji2023investigating}. %\jessy{there's a dependabot study that can be referenced here}

Listing participants use different mediums to let the community know about the need to upgrade, which include sending messages to mailing lists and backchannels ($L=7$), creating GitHub security advisories ($L=6$), and in some cases, quickly requesting a CVE ($L=5$). Interviewee participants were also wary of making sure users are aware of vulnerabilities ($I=7$), two of which felt that creating a CVE is enough to ensure visibility to users and dependents. One interviewee felt that disclosure is only necessary when a vulnerability is particularly important because there is \textit{``a lot of bandwidth on security disclosures to begin with.''} (P6).

\vspace{0.1cm}

\noindent\textbf{Security policies }
The next most listed current practice used is having a project security policy ($L=37, I=10$). OSS security policies have mostly been used to inform reporters how to properly communicate vulnerabilities to maintainers via security contact~\cite{wermke2022qual-OSSP}, but they are generally underused~\cite{ayala2023workflowssps}. 

Although most listing participants mention using security policies to simply provide a security contact ($L=11$), in some cases, maintainers link an organization-specific security policy published outside of GitHub ($L=3$). One interviewee mentioned how they use security policies to explicitly discourage contributors from reporting vulnerabilities publicly and provide multiple methods of private communication:

\leftskip=0.5cm\rightskip=0.5cm

\noindent\textit{``We have a security policy in place where we say please do not report it publicly but try to contact me personally via email or send a mail to our security mailing list or create a security advisory on GitHub.''} (P13).

\leftskip=0cm\rightskip=0cm

\vspace{0.1cm}

\noindent\textbf{Private vulnerability reporting }
Another GitHub platform security feature listing participants mentioned frequently is private vulnerability reporting ($L=20, I=9$). This particular feature allows contributors to privately report vulnerabilities within the GitHub platform. OSS maintainers can then review a report with functionalities to update its severity, invite others to develop a fix, and decide whether or not to request a CVE. 

Listing survey participants and interviewees mention using the private forks from private vulnerability reporting to quietly develop fixes ($L=6, I=7$). Four interviewees mentioned how they like this feature because it provides an easy method of reporting security bugs and is quick to set up, i.e., by clicking enable. One interviewee describes private vulnerability reporting as \textit{``very comfortable and very easy to use.''} (P9). Others expressed satisfaction with private vulnerability reporting because everything is in a central space ($I=2$), i.e., submitted reports are contained in GitHub.

\vspace{0.1cm}

\noindent\textbf{Automation tooling }
Another method of current practices listing and interviewees mention is the usage of automated dependency analysis tooling and code scanning $(L=16, I=12)$. Dependency analysis provides alerts of library upgrades, e.g., patched versions, while code scanning can reveal vulnerabilities, e.g., secrets, as a result of running static analysis.

Listing participants and interviewees mentioned using Dependabot as a primary source of upgrading dependencies ($L=12, I=6$). Others mentioned using the Renovate bot that can allow dependencies to be auto-merged if there are no code conflicts ($L=4, I=3$), reducing manual overhead:

\leftskip=0.5cm\rightskip=0.5cm

\noindent\textit{``The first one that I use quite often is Renovate, that is a tool in Github easily available where you can configure: I want this and this upgraded like that, and you can have all kinds of settings and then it's automatically gives you a pull request [...] with a dependency update and automatically, the test pipeline fires.''} (P1).

\leftskip=0cm\rightskip=0cm

However, participants describe how platform security features, which are recommended for effective vulnerability management, pose still too much manual effort (Section~\ref{sec:psfchallenges}).

\vspace{0.1cm}

\noindent\textbf{GitHub Issues }
Some listing participants and interviewees indicate using GitHub issues for reporting vulnerabilities ($L=9, I=6$). When a GitHub Issue is submitted, it is publicly accessible in the Issues tab located at the top of the project landing page. 

Two listing participants in particular do not mind having vulnerabilities being reported publicly because of visibility, while one listing participant described how they use \textit{``the same public PR process I use for any other issue.''} One interviewee described how they do not mind using GitHub issues when a security bug is not determined to be severe to get help from the public, while another interviewee explained their rationale: 

\leftskip=0.5cm\rightskip=0.5cm

\noindent\textit{``If somebody reports a security issue [publicly], I don't really see a problem with it. Obviously it can be problematic, but I don't really care that much about how it is reported as long as I fix it in a short time.''} (P19).

\leftskip=0cm\rightskip=0cm

\vspace{0.1cm}

%These perspectives reflect that while public issue reporting can enhance transparency and community support, private methods might still be preferred for handling more severe vulnerabilities, especially for projects gaining popularity.

\noindent\textbf{Ignoring vulnerabilties }
Two listing participants mention how they ignore vulnerabilities. One attributed this behavior to a lack of motivation for setting up any security features or tooling and indicated that \textit{``financial support or sponsorship''} would be most beneficial for them to improve their vulnerability management practices. The other respondent listed \textit{``unless the project is extremely sensitive - avoid implementing any policy''} and expressed the perception that having security features enabled for projects is unnecessary. Though this respondent listed that they were interested in participating in our interview study, they did not respond with any contact information or reach out to us directly. 

\subsection{Challenges with vulnerability management}\label{sec:genchallenges}

All interviewees described wearing many hats when it comes to OSS maintenance, some of who are lone maintainers ($I=11$).
General vulnerability management challenges OSS maintainers face range from trusting the software supply chain to lack of time and resources to issues with CVEs.
%Many participants noted how bug bounty reports are just security-oriented pull requests. 
Participants also describe how a lack of standardized vulnerability handling procedures and implementing proper coordinated disclosure are prominent challenges.
Some bring up the idea of having \textit{``imposter syndrome''} when receiving vulnerability reports, while others share experiences of negative encounters with reporters and companies. 

\noindent\textbf{Supply chain trustworthiness }
Supply chain trust was the most listed challenge with vulnerability management ($L=36, I=6$). Use cases and duties related to the software supply chain in OSS include adopting upstream dependencies, tracking the status of dependencies, and updating dependencies in a timely manner, e.g., when a vulnerability is patched.

Specific challenges that the participants mentioned include the burden of keeping updated with dependencies and the latest vulnerabilities ($L=20$) and dealing with unmaintained dependencies or delays in pushing a vulnerability fix ($L=12$), which can be time-consuming and resource-intensive. 
One interviewee was particularly concerned about scenarios \textit{``where people purposefully like to put security vulnerabilities into [OSS projects]''} (P6), highlighting the risk of malicious actors deliberately introducing vulnerabilities into upstream dependencies, e.g., the \code{xz-utils} incident (CVE-2024-3094)~\cite{xzutils}.

\vspace{0.1cm}

\noindent\textbf{Lack of understanding }
The second most listed challenge for conducting vulnerability management is a lack of understanding ($L=35, I=12$). 
Not being able to effectively understand reported vulnerabilities can lead to delays in patching and disclosure to affected dependent client projects.

Factors reported affecting a lack of understanding include complexity ($L=19, I=4$), developing a patch ($L=7, I=7$), testing ($L=6, I=6$), and knowledge gaps ($L=5, I=8$). 
One participant listed that \textit{``some vulnerabilities can be complex and require extensive investigation and testing to ensure they are fully resolved without introducing new issues,''} reflecting platform security feature challenges we explore in Section~\ref{sec:psfchallenges}, while one interviewee said \textit{``my brain is far too small to understand [vulnerabilities]''} (P9). We explore potential avenues maintainers believe OSS platforms can take to minimize such knowledge gaps and awareness in Section~\ref{sec:psfwants}.

\vspace{0.1cm}

\noindent\textbf{Lack of time and resources }
The next most listed software vulnerability management challenges are the lack of time ($L=25, I=9$) and resources ($L=23, I=11$). The time OSS maintainers spend on developing and managing projects is limited, e.g., hobbyists. Further, resources are scarce, e.g., large-scale software ecosystems like Python Package Index and NPM are primarily made up of projects with a single maintainer~\cite{npmgraph,pypigraph}.

Challenges associated with a lack of time and resources include balancing prioritizing vulnerabilities with ongoing development tasks ($L=21, I=16$), the ability to triage reports promptly ($L=15, I=11$), and getting help from others ($L=8, I=5$). One interview participant summarizes:

\leftskip=0.5cm\rightskip=0.5cm

\noindent\textit{``While I prioritize addressing vulnerabilities immediately, balancing this with ongoing development tasks can sometimes be challenging [...] There are limited resources and time available to address every reported vulnerability quickly.''} (P17).

\leftskip=0cm\rightskip=0cm

\vspace{0.1cm}

\noindent\textbf{Negative relationships with CVEs }
Participants also expressed bad relationships with CVEs and the overall CVE process as a challenge when conducting vulnerability management ($L=8, I=9$). 
CVEs play an important role in the overall disclosure process and help promote transparency in the OSS ecosystem, e.g., upgrade notifications. 

One listing participant explains their stance on CVEs: 

\leftskip=0.5cm\rightskip=0.5cm
\noindent\textit{``The CVE program suffers from many single points of failures: managed by the USA (not 24/7) hence a CVE ID cannot be delivered fast. CISA analysts backlog and [don't] have enough time and understanding of the system's complexity to properly analyze reports; thus, publish poor quality content. The whole process is outdated and must be reformed to a distributed approach to enable international sources of trust to work.''}

\leftskip=0cm\rightskip=0cm

Others described experiences where fixes were put on hold because of pending CVEs ($L=3$) or feel intimidated by the nature of CVEs ($L=2,I=2$). In particular, one interviewee described their negative perception of CVEs and observation of other project maintainers' handling of CVEs:

\leftskip=0.5cm\rightskip=0.5cm

\noindent\textit{``I'm incentivized to lie to make the CVE [severity] lower because it makes my project look bad, you have to be really, really honest [...] I noticed a lot of people like downgrade their CVEs.''} (P15).

\leftskip=0cm\rightskip=0cm

This quote highlights potential ethical dilemmas and pressures faced by OSS maintainers when dealing with CVEs, which can negatively affect the accuracy and reliability of severity metrics throughout the OSS ecosystem.

\noindent\textbf{Lack of procedures and coordinated disclosure }
Though established procedures can help alleviate the receive-to-resolve timeline, the lack of procedures is a challenge OSS maintainers also face ($L=7, I=5$). Further, participants also express challenges with being able to effectively reach affected dependent client projects and users ($L=7, I=4$).

OSS maintainers express a lack of recommended standardized processes for handling vulnerabilities ($L=5, I=1$) due to limited experience ($L=2$), some even feeling intimidated ($L=2$). 
Two interviewees described a sense of imposter syndrome when receiving vulnerabilities because \textit{``there are so many things we need to watch out for, it's hard to stay confident that you're doing the right thing.''} (P13). 
Further, participants expressed concerns about effectively disclosing the nature of the vulnerabilities ($L=4, I=7$) and a sense of mistrust with upstream projects not disclosing vulnerabilities properly ($L=2, I=2$). 
These perspectives suggest needs for clearer guidelines and better support for OSS maintainers in handling vulnerabilities, reported in Section~\ref{sec:discussion}, as well as further research on the adoption of and improving attestation practices, e.g., software-bill-of-materials, to foster upstream trust within the software supply chain~\cite{donoghue2024sbom,xia2023sbom,nocera2023sbom}.

\vspace{0.1cm}

\noindent\textbf{Negative attitudes }
The least listed challenge of vulnerability management is negative attitudes from reporters ($L=6,L=9$). The OSS ecosystem is human-centered, e.g., through community and collaboration, and is not a stranger to toxic interactions~\cite{raman2020burnout,miller2022did}. One interviewee described experiences with companies demanding pentests. Participants mention the argumentative nature with vulnerability reporters ($L=3, I=7$) and those with sole intentions to make money ($L=3, I=5$).

\leftskip=0.5cm\rightskip=0.5cm

\noindent\textit{``They give me this list of vulnerabilities in an email and then say, we're going to make it public in a week. And I think it's not so bad to make it public; in fact, both times I said go ahead and make it public right now. But the way people give you this problem and say fix it or else, it's not a very conducive environment.''} (P2).

\leftskip=0cm\rightskip=0cm

\subsection{Challenges with platform security features}\label{sec:psfchallenges}

The adoption of platform security features (PSFs) promotes a robust vulnerability management process, especially if they are usable for OSS maintainers without a security background. 
In this section, we report various challenges and first-hand experiences as a result of adopting such features, revealing why some maintainers may choose to disable them as a result. 

\vspace{0.1cm}

\noindent\textbf{Not enough automation }
The most listed PSF challenge described is that there is not enough automation ($L=39, I=11$). 
As described earlier in Section~\ref{sec:genchallenges}, OSS maintainers have limited time and resources to address every reported vulnerability quickly.
Automation for security-oriented tasks helps promote easy security without additional overhead.

Participants express challenges regarding automation to update dependencies ($L=24, I=7$). In particular, five interviewees are okay with auto-merging dependency upgrades as much as possible, while others would prefer to do so on a library-by-library basis ($I=2$). One interview participant mentioned auto-merging private vulnerability report fixes if the build does not break; however, private forks do not have CI integration and participants describe experiences with broken builds and tests, which we report later in this section.

One interviewee describes how they are okay with merging automated pull requests regardless of testing: \textit{``Go ahead and merge the PR. I don't even really test it.''} (P5). This perspective reflects a desire for streamlined processes, even if it comes at the cost of rigorous testing, underscoring the tension between automation convenience and careful oversight needs.

\vspace{0.1cm}

\noindent\textbf{Too much noise and vulnerability scoring issues }
Listing participants mentioned that too much noise from PSFs ($L=24, I=10$) and issues from vulnerability scores ($L=21, I=9$), e.g., inaccuracy, are particularly challenging to deal with. Participants describe noise as many false alarms, different from spam or low-quality reports, and how noise can take time away from general OSS tasks and in some cases, overwhelm or scare OSS maintainers ($L=4, I=6$). 

It is common knowledge that noises from dependency management~\cite{mirhosseini2017can,he2023automating} and static analysis~\cite{wedyan2009effectiveness,johnson2013don} tools are problematic.
A majority of noise mentioned is from dependency false positives ($L=8, I=6$), while others said it is from static analysis tooling ($L=4, I=2$), e.g., code scanning, and a general sense of annoyance from notifications ($L=2, I=2$). One interviewee mentioned how even proprietary scanners produce too much noise -- we report remediations to help improve PSF setup and reduce noise in Section~\ref{sec:psfwants}. Two interviewees mentioned how noise negatively impacts their motivation to continue maintaining OSS projects, one described:

\leftskip=0.5cm\rightskip=0.5cm

\noindent\textit{``I left this project, I'm not doing this anymore [...] I think there's a lot of noise [...] and then the dedication, the love and the passion, the patience, going over it, and taking care of it, it's not easy at all. So security is kind of a second thought to most of us.''} (P8).

\leftskip=0cm\rightskip=0cm

In addition to noise, participants describe issues with vulnerability scores from reported vulnerabilities, e.g., CVE scores are inflated ($L=5, I=4)$ and unsure how to correctly calculate or adjust CVSS scores ($L=3, I=8$). One interview participant summarizes their past experiences with attempting to properly calculate security metrics:

\leftskip=0.5cm\rightskip=0.5cm

\noindent\textit{``I always have issues with calculating CVSS [scores]. All the documentation I found seems to be like for security researchers, or people who have experience with security incidents. There's nothing that just describes it in everyday terms that I can really wrap my head around, so that's one of the biggest difficulties.''} (P3).

\leftskip=0cm\rightskip=0cm

\vspace{0.1cm}

\noindent\textbf{Absent CI processes in private forks, failing tests and broken builds in the public eye }
The next most listed challenge with PSFs is the lack of CI processes when developing fixes on a private fork ($L=8, I=7$), i.e., as a result of adopting the built-in private vulnerability reporting feature. Although private forks are a recommended method of working on fixes with reporters, not being able to run CI processes on such fixes in the same environment as merging pull requests on the main branch can be problematic, resulting in overhead.

To get around the lack of CI processes in private forks, participants have resorted to hosting additional private repositories outside of GitHub that mimic their public presence ($L=2, I=1$) or running potential fixes through build processes on personal machines ($I=4$). 
Both of these solutions, while functional, introduce additional challenges and complexities, e.g., maintaining parallel environments and ensuring consistency across different setups.
One interview participant described an elaborate approach: 

\leftskip=0.5cm\rightskip=0.5cm

\noindent\textit{``We have [someone], our traffic controller, and their role is to check that the incoming security reports [...] If they consider it something we need to be concerned with, they create an issue in a private project [...] It really slows the process down, because we have to merge one patch, then we have to go to our repo, pull in commits to the new one we need to release.''} (P14).

\leftskip=0cm\rightskip=0cm

Participants report experiences of failed tests or broken builds after patches are merged to the main public repository ($L=6, I=7$), so OSS maintainers must thoroughly ensure fixes do not introduce new issues. 
\textit{``The biggest problem for us is the fact we can't run our automated tests on the fixes that we make on those forks.''} (P14).
This emphasizes a development workflow issue caused by the lack of automated testing capabilities in private forks, which is crucial for program repair and preventing regressions -- a current multi-dimensional and challenging research area~\cite{kabadi2023apr,bui2024apr,minhas2023regression}.%fu2022vulrep,minhas2023regression,brahneborg2017regression}.

\vspace{0.1cm}

\noindent\textbf{Cluttered notifications, setup and usage is too manual }
The least listed PSF challenges are cluttered notifications ($L=4, I=4$) and too much manual effort ($L=3, I=3$), i.e., usability challenges.
Interviewees describe that the best security is \textit{``easy security''} ($I=6$), including the ease of use for PSFs. When security features are user-friendly and require minimal effort to manage, they can be effectively utilized by OSS maintainers without additional overhead.

Participants describe how dependency notifications are too cluttered ($L=2, I=3$), and how there should be a merge-all button, i.e., to reduce manual effort, for dependency upgrades that do not cause merge code conflicts ($L=1, I=3$). %One interviewee describes such clutter:

\leftskip=0.5cm\rightskip=0.5cm

\noindent\textit{``They are all grouped together at the bottom of your notification panel and they appear only if all the others are marked as done [...] just terrible to deal with [...] There is like a cron job that runs then delivers you all of those once a week, they're all bundled.''} (P10).

\leftskip=0cm\rightskip=0cm

Other tasks described as too manual by interviewees include having to individually enable PSFs for each project ($I=4$), e.g., as opposed to a centralized approach where all projects are presented on a single screen, and having to manually add the same collaborators to a private fork every time a vulnerability is privately reported ($I=3$). 

\subsection{Barriers hindering adoption of platform security features}\label{sec:psfbarriers}

Despite the importance of actively practicing secure coding practices and being knowledgeable about general security concerns, OSS developers typically do not have a security background.
A majority of our participants also lack such background ($L=50,I=15$). 
In this section, we report possible barriers that hinder PSF adoption, including lack of awareness, complex setup procedures, concerns about project reputation, and perceptions that they are unnecessary.\\

\vspace{-0.3cm}

\noindent\textbf{Lack of awareness and bad UI presentation }
The most listed PSF barrier is lack of awareness ($L=33, I=12$). PSFs are available for usage so that OSS projects can have robust vulnerability management processes and proper disclosure upon vulnerability patching. This lack of awareness implies that although tools and processes are available to help promote a thriving secure OSS ecosystem, they are underutilized as indicated in prior work measuring OSS PSFs' usage~\cite{ayala2023workflowssps}.% and in our recruitment pool statistics from~\autoref{tab:svmusage}.

Participants mentioned how they were not aware of security policies ($L=43, I=8$), private vulnerability reporting ($L=43, I=10$), and public security advisories ($L=34, I=4$) or the GitHub advisory database ($L=13, I=6$).
Further, 26.7\% (21/80) of listing participants indicated that they have none of the three previously mentioned PSFs enabled.  
One interviewee expresses how \textit{``the main problem is just that many people don't know about it''} (P18), and another interviewee, who has had eight CVE-assigned vulnerabilities in a project they manage, expressed curiosity after learning about what private vulnerability reporting has to offer:

\leftskip=0.5cm\rightskip=0.5cm

\noindent\textit{``It's on my list to actually research now. Yeah, it looks like they've got a pathway to disclosure in CVEs that's integrated and seems like a good tool for us.''} (P20).

\leftskip=0cm\rightskip=0cm

Related to lack of awareness, bad UI presentation is another PSF barrier participants mentioned ($L=8, I=6$). In particular, participants feel that PSFs are too hidden or hard to find ($L=5, I=6$) and that there are just too many features to potentially configure ($L=2, I=3$). One interviewee described how PSFs feel like \textit{``second-class features''} (P10). This perception can discourage maintainers from exploring PSFs' capabilities, further contributing to their underuse.

\leftskip=0.5cm\rightskip=0.5cm

\noindent\textit{``I mean, I'm just looking at how to or for a way to roll stuff out, but it's pretty hidden. I can roll out a policy that allows private vulnerability and a lot of other stuff, but you have to really click through and find it.''} (P11).

\leftskip=0cm\rightskip=0cm

\vspace{0.1cm}

\noindent\textbf{Complex to set up or use, not sure what they do }
Listing participants mentioned that PSFs are too complex to set up or use ($L=26, I=7$). Though not nearly listed as much, participants are \textit{``not sure what they do in the first place''} ($L=4, I=2$). These perceptions reflect a barrier of adoption since OSS maintainers question their overhead and purpose.
Interviewees express a sense of excessive overhead with setting up PSFs ($I=4$). 
Others cite general ignorance as to why they are not aware of what particular PSFs do ($L=3, I=7$). 
As a result, they did not bother looking into PSFs.
If users are unclear about what these features do or how they are able to benefit their projects, they are less likely to invest effort in setting them up, especially if they are perceived as complex.

\leftskip=0.5cm\rightskip=0.5cm

\noindent\textit{``The biggest reason I never used them is they've never been pushed or the benefits of them sold to me [...] If it's really easy and simple to use, it'd be nice if that is kind of turned on by default on all projects.''} (P12).

\leftskip=0cm\rightskip=0cm

Participants also reference previous experiences with trying out PSFs but refuse to look into additional offered tooling because of usage complexity ($L=11, I=4$), e.g., with dependency graphs ($L=2$). These insights suggest simplifying the setup process and providing clearer information about the purpose and use of PSFs for OSS maintainers looking to adopt them to manage vulnerabilities.\\

\vspace{-0.3cm}

\noindent\textbf{Perception that they are unnecessary }
The next most listed PSF adoption barrier is the perception that they are unnecessary ($L=23, I=6$). When OSS maintainers perceive PSFs as not adding value to their current processes, they will likely refrain from investing additional time and resources into learning about or implementing these tools; thus, undermining recommended efforts to promote a secure OSS ecosystem.

Participants mention how PSFs are unnecessary for a variety of reasons, including the perception that projects lack importance ($L=16, I=6$), adding PSFs is overkill ($L=5, I=3$), or that maintainers do not value security ($I=2$). These perceptions highlight a need for more documentation on the value of security measures ($L=17, I=8$) and mechanisms for PSFs to be tailored to fit specific project needs and scale.

\leftskip=0.5cm\rightskip=0.5cm

\noindent\textit{``I haven't really needed anything more involved than GitHub issues [...] Security isn't something that we worry too much about. We're not ready to hear that message, even if GitHub does push me, I'll probably just skim over them, because I'm not ready to actually to, you know, get that message [...] We worry, we kind of have it in mind, but it's not our main goal.''} (P8).

\leftskip=0cm\rightskip=0cm

\vspace{0.1cm}

\noindent\textbf{Project reputation and a lack of motivation }
The remaining barriers to PSF adoption OSS maintainers mention are concerns with project reputation ($L=11, I=4$) and a lack of motivation ($L=5, I=4$). Concerns about maintaining a positive public perception can deter OSS maintainers from implementing PSFs, that would otherwise enhance security, while those without motivation to adopt PSFs may deprioritize or ignore the use of PSFs.
The attitude concerning reputation is not unique to maintainers. Alomar et al.~\cite{alomar2020you} observed this attitude at the organizational level, where organizations try to lower the severity ratings of vulnerabilities in their products.

Participants point out fear of negative project reputation as a reason to not adopt PSFs ($L=3, I=3$), e.g., owning a project with previous high or critical CVE-assigned vulnerabilities ($I=1$). On the other hand, some interviewees consider a project without vulnerabilities as suspicious ($I=2$), i.e., patched vulnerabilities are a good sign of a ``healthy project'' (P14). One interviewee reflected on such dilemma:

\leftskip=0.5cm\rightskip=0.5cm

\noindent\textit{``It's always in the back of my mind when looking at an issue and seeing, should this go through the security advisory process? Or should it just be a normal PR and fix? That's the end of it. But that's wrong, and I know it. It still feels like, you know, hurting the reputation of my project. But it's wrong, I know it.''} (P3).

\leftskip=0cm\rightskip=0cm

When it comes to lack of motivation, participants cite ``maintainer burnout'' as the primary reason for not wanting to deal with vulnerabilities ($L=3, I=4$). This burnout can lead to a reduced willingness to engage with vulnerabilities, as maintainers may already be overwhelmed by other OSS tasks, e.g., high-stress levels from frequent demands for features and bug fixes ~\cite{raman2020burnout}. Further, others see no benefit for improving project reputation through a security lens ($L=1, I=2$), leading them to deprioritize or disregard the adoption of PSFs.

\vspace{-0.2cm}

\subsection{Opportunities for improvement \& support}\label{sec:psfwants}

Lastly, we asked participants about success stories or positive outcomes as a result of their continuous vulnerability management efforts, if applicable, as well as supplemental features or improvements to current PSFs that would benefit their current vulnerability management approaches the most.

\vspace{0.1cm}

\noindent\textbf{Assisted vulnerability analysis and triaging }
Participants expressed the most need for assisted vulnerability analysis and triaging ($L=39, I=9$), i.e., via automation mechanisms. 
In particular, participants felt that this would be useful for understanding vulnerabilities and their actual impact on OSS projects ($L=34, I=7$) to reduce false positives and noise described in Section~\ref{sec:psfchallenges}, e.g., \textit{``I hope a tool can take a context into consideration and it should help tooling avoid the false positives, and to trigger only this stuff when [vulnerable]''} (P7).
Further, participants express a need for assistance with developing fixes and generating tests ($L=21, I=6$), which could streamline the remediation process and ensure more effective vulnerability management, e.g., \textit{``generate, you know, tests with test cases or something like that, maybe as a way to lighten the burden of actually developing tests''} (P5). 

\vspace{0.1cm}

\noindent\textbf{PSF setup assistance, checklists, and nudges }
Participants also showed interest in having assisted PSF setup ($L=37, I=10$). 
In particular, interviewees mention needs for assistance generating security policy content using project scope ($I=3$), security tooling recommendations based on project contents ($I=6$), and interactive guidance throughout the setup process ($I=7$), e.g., \textit{``it's a little bit not easy to use [...] now I need to figure out, okay, what is the proper setup for my project [since] I'm of the mindset that brevity is king.''} (P9). 
Further, participants mention wanting checklists and suggestions of things to do for recommended PSFs ($L=15, I=3$), alongside nudges or reminders and ``easy'' configurations as methods of encouraging others to strengthen their projects' security posture ($L=16, I=5$). One interview elaborates on their view of overall PSFs: \textit{``It's pretty overwhelming, and you might just be like, why do I need any of these? Like, why is this important? Having a single button that just says, enable best practices, would go a long way.''} (P16). 

\vspace{0.1cm}

\noindent\textbf{Security funding and cyber defense gamification }
The next most-listed want for participants is security-specific funding ($L=32, I=7$), i.e., funding to be used for security-related tasks and efforts. 
In particular, participants mention using funds for maintainers and reporters to get paid ($L=18, I=6$), funding a dedicated bounty pool for valid vulnerabilities ($I=3$), or requesting annual reviews from security experts ($I=2$). 
%%%\textit{``I'm a bit concerned that if I open a door on GitHub for people to report vulnerabilities, I'm a little bit scared that they will ask something in return and I will not be able to compensate them.''} (P22).
There was also interest in cyber defense gamification ($L=13, I=6$), i.e., to recognize projects that adopt vulnerability management processes. 
Four interviewees mention how they use reporter reputation to determine vulnerability report legitimacy. 
Such participants and others expressed interest in project reputation icons, e.g., a \textit{``green shield''} ($I=3$), for projects that adopt recommended PSFs and tooling  ($I=7$); thus, recognizing and rewarding projects that exhibit a proper security posture. %%%One interviewee describes their perspective: 
\textit{``Everyone wants to have the green shield [...] This community health status people see, stuff like that, like you'll be surprised by how many people want to feel those bars.''} (P10). 
%%%Trockman et al.~\cite{trockman2018adding} previously speculated on using gamification for bug fixing.

\vspace{0.1cm}

\noindent\textbf{User-friendly resources and documentation }
Lastly, participants expressed interest in having more user-friendly documentation and resources ($L=17, I=8$), some citing general \textit{``ignorance''} of proper OSS security ($I=6$). 
In particular, participants mention OSS recommended training material for \textit{``normie developers''} ($L=3, I=4$), e.g., free webinars ($I=2$), redirection to related projects with implemented security practices ($L=7, I=3$), and \textit{``easier directions''} for setting up and what to expect from PSFs ($I=6$), e.g., not being \textit{``scared''} of false positives ($I=3$). 
\textit{``Security best practices and tooling and all of that is tribal knowledge, and it shouldn't be.''} (P12).
